Evaluating two-loop non-planar master integrals for Higgs + jet production with full heavy-quark mass dependence

We present the analytic computation of a family of non-planar master integrals which contribute to the two-loop scattering amplitudes for Higgs plus one jet production, with full heavy-quark mass dependence. These are relevant for the NNLO corrections to inclusive Higgs production and for the NLO corrections to Higgs production in association with a jet, in QCD. The computation of the integrals is performed with the method of differential equations. We provide a choice of basis for the polylogarithmic sectors, that puts the system of differential equations in canonical form. Solutions up to weight 2 are provided in terms of logarithms and dilogarithms, and 1-fold integral solutions are provided at weight 3 and 4. There are two elliptic sectors in the family, which are computed by solving their associated set of differential equations in terms of generalized power series. The resulting series may be truncated to obtain numerical results with high precision. The series solution renders the analytic continuation to the physical region straightforward. Moreover, we show how the series expansion method can be used to obtain accurate numerical results for all the master integrals of the family in all kinematic regions.

==> expansionmethodsection.tex <==
In this section we describe a strategy based on (generalized) series expansions by which the differential equations satisfied by Feynman integrals may be solved. By truncating the series to arbitrarily high orders, this allows to obtain numerical values with arbitrary precision, in all kinematic regions. The strategy may be employed to compute both the polylogarithmic and the elliptic sectors, and will be described more exhaustively, together with an application to the planar families of Higgs + jet in the physical region, in \cite{moriello_expansions}. Here we will content ourselves with
illustrating the general idea, and how it applies to our particular case. Similar methods were used for single-scale problems in \cite{Pozzorini:2005ff,Aglietti:2007as,Lee:2017qql,Lee:2018ojn,Bonciani:2018uvv,Mistlberger:2018etf}.

Given a collection of master integrals $\vec{\text{I}}$, our solution strategy consists of four steps:
\begin{enumerate}
  \item Obtain an expression with \emph{arbitrary numerical precision} $\vec{\text{I}}(x_0)$ for the integrals at (or in the asymptotic limit of) a given kinematic point $x_0$.
  \item Write down the differential equations $\partial_\lambda \vec{\text{I}}(x(\lambda)) = \mathbf{A}(\epsilon,\lambda) \vec{\text{I}}(x(\lambda))$ for the integrals along a line (or any other path) $\gamma(\lambda)$ joining the original boundary point $x_0$ to any other point $x_1$ of interest.
  \item Write the solution of the differential equations using (generalized) power series.
  \item Obtain the values $\vec{\text{I}}(x_1)$.
\end{enumerate}
A few comments are in order for each of the steps above.

1) The expression $\vec{\text{I}}(x_0)$ must allow a numerical evaluation with arbitrary precision. This might be achieved either by a closed formula such as those provided for the heavy mass limit in section \ref{sec:boundaryterms}, but also by the outcome of the expansion method itself: a representation of $\vec{\text{I}}(x_1)$ as a series expansion truncated at an arbitrarily high order (and thus with arbitrary precision). We stress that $x_0$ could be either a regular point or a singular point. In the case of a regular point we obtain an ordinary power series, on the other hand for a singular point we obtain a generalized power series with non integer powers and logarithms.

2) In the second step, one is in principle allowed to choose any path $\gamma(\lambda)$, but in practice we find it convenient to choose a straight line \footnote{One might wonder if, depending on the situation, choosing some curved path might be more convenient because it might allow to rationalize some of the square roots of the problem. However, as it should be clear by the end of the section, the power of the expansion method relies on the fact that one treats in the same way situations with rational functions and algebraic functions, so that rationalization of square roots is not necessary nor helpful.}, i.e. $\gamma(\lambda) = x_0 (1-\lambda) + x_1 \lambda$. %The only restriction is that the path must not cross any singularity of the integrals, such as $s=4 m^2$. Spurious singularities - singularities of the differential equations which are not expected, on physical grounds, to be singularities of the integrals - are in principle not a problem.
%However, to guarantee a fast convergence of the series expansion we find more convenient to treat them as true singularities.
Special attention must be payed to the radius of convergence of the series of the third step: to guarantee a sufficiently fast convergence it is in practice necessary to choose a point $x_1$ not too far from $x_0$, since the path $\gamma$ will (likely) cross a physical singularity after $x_1$, thus the series expansion will break there and converge poorly nearby. A good choice is to pick $x_1$ halfway between $x_0$ and the first singularity met along $\gamma$. %Finally let us point out that one has to take into account the singularities located at negative values of the expansion parameter, that is for $-1<t<0$, since they affect the radius of convergence as well.

3) Upon choosing a path $\gamma$ the problem is reduced to one dimension, and the differential equations are in the single variable $\lambda$ parametrizing the path, which we solve in terms of power series. % We would like to emphasize that, even if the expansion point $x_0$ is a (regular)\footnote{In Feynman integrals, we do not expect the occurrence of  essential or irregular singularities, such as $\exp(1/x)$ or $\exp(1/\log(x))$, for which these methods do not apply.} singular point, these methods apply. 
This strategy applies to differential equations of arbitrary order in a single unknown function, so when necessary we decouple the system $\partial_\lambda \vec{\text{I}}(\lambda) = \mathbf{A}(\epsilon,\lambda) \vec{\text{I}}(\lambda)$ by taking higher derivatives until we can write a single differential equation for each integral. In order to solve the equations we first series expand $\mathbf{A}(\epsilon,\lambda)$ around a regular or singular point. The series solution is then obtained by integrating order-by-order in epsilon the (expanded) differential equations.  At any given time one has to perform only integrals of the form,
%$$\int t^q\  \mathrm{log}(\lambda)^n\  d\lambda = (-1)^n (1+q)^{-(n+1)}\Gamma(1+n,-(1+q)\mathrm{log}(\lambda))\quad  q \in \mathbb{Q}\,,\ n \in \mathbb{N}, $$
\begin{align}
\int t^c  \log (\lambda)^n\  d\lambda  \quad  c \in \mathbb{C}\,,\ n \in \mathbb{N}, \nonumber
\end{align}
which can be done analytically, and which are themselves expressed in terms of functions of the form $t^c \, \log (\lambda)^n$. This is the case regardless of the details of the differential equations, and in particular of the presence of algebraic functions.
Finally, the series solutions to the differential equations depend on a number of integration constants, which have to be fixed matching the boundary conditions at $x_0$. 

4) Having obtained a numerical expression for $\vec{\text{I}}(x_1)$, whose precision can be increased by increasing the order at which the series are truncated, one can iterate the procedure to reach any point in the kinematical space. The paradigmatic example is the crossing of a physical singularity. For example, suppose that somewhere along the line $\gamma$ joining $x_0$ and $x_1$ there is a point $x_{\mathrm{sing}}$ where some Feynman diagrams develop a singularity. In this case, we first write an expansion from $x_0$ to $x_{\mathrm{sing}}$, which allows to obtain an analytical expression for the diagrams at the midpoint of this interval. We use these values to fix the constants of integration in the expansion around $x_{\mathrm{sing}}$ provided by the Frobenius method. After an analytic continuation of the latter expansion, we obtain the desired values at $x_1$. Clearly, the procedure (which also solves the problem of the radius of convergence) can be carried over to reach any point in any sheet of the kinematic space. For phenomenological purposes however, we are just interested in reaching one point in the physical region. %From there, in principle, we do not need to cross any other physical singularity to reach any other point of interest, instead it suffices to patch together expansions at regular point which in practice are easier to do.

Before ending this section we give some further details regarding the analytical continuation. Suppose that the expansion point $x_0$ is singular, for example corresponding to a physical singularity such as $s = 4 m^2$, and that the path parameter $\lambda$ is positive for $s \le 4m^2$. The series will contain terms with powers of $\log(\lambda)$ and half-integer powers $\lambda^{n/2}$, which must be analytically continued past the singularity, i.e. for negative values of $\lambda$. Following the Feynman prescription this is done by giving small imaginary parts $i\epsilon$ to Mandelstam variables and masses, which implies that we continue $\log(\lambda)$ to $\log(-\lambda)-i \pi$ and $\lambda^{n/2}$ to $(\lambda)^{n/2}.$

%In the next section, we will illustrate how the above method unfolds in the case at hand. We will first study the differential equations for the elliptic sectors and motivate the choice of a better basis, then we will present the iterative algorithm which implements the expansion method, and finally present our results in the form of plots.



